Report of the Topical Group on Cosmic Frontier 5 Dark Energy and Cosmic Acceleration: Cosmic Dawn and Before for Snowmass 2021

This report summarizes the envisioned research activities as gathered from the Snowmass 2021 CF5 working group concerning Dark Energy and Cosmic Acceleration: Cosmic Dawn and Before. The scientific goals are to study inflation and to search for new physics through precision measurements of relic radiation from the early universe. The envisioned research activities for this decade (2025-35) are constructing and operating major facilities and developing critical enabling capabilities. The major facilities for this decade are the CMB-S4 project, a new Stage-V spectroscopic survey facility, and existing gravitational wave observatories. Enabling capabilities include aligning and investing in theory, computation and model building, and investing in new technologies needed for early universe studies in the following decade (2035+).

==> TtoO.tex <==
\section{From Theory To Observations}
\label{sec:TtoO}

\subsection{Primordial Structure, \textcolor{red}{dan, adrian, laura 5 pages}}
\label{sec:pStruc}

Structure in the universe is believed to have originated during inflation from quantum fluctuations of the inflaton or, equivalently, the scalar mode of the metric. These fluctuations change the amount of inflation that occurred in different parts of the universe, and thus correspond to a change in the physical energy densities from place to place.  After reheating, these density perturbations grow and evolve as the re-enter the cosmic horizon.  The different components of the energy density and their fundamental interactions shape this subsequent evolution, giving rise (at linear order) t
\beq
\delta_{i}(\vec k,z) = T_i(k,z) \zeta(\vec k)
\eeq
where $\vec k$ is a comoving wave-number, $k= |\vec k|$, $\zeta(\vec k)$ is the scalar metric fluctuation, $\delta(\vec k,i)$ is the density contrast of species $i$ and $T_i(k,i)$ is its transfer function.  

Measurements of the statistical properties of these densities encode both the physics of inflation and of the evolution of the universe after the hot-bang bang.  For example, the total matter power spectrum, 
\beq
P_{m}(k,z) = T^2_m(k,z) P_\zeta(k) \ ,
\eeq
is both a measurement of the power spectrum from inflation, $P_\zeta(k)$, and the growth of structure, BAO, etc. through the transfer function $T_m(k,z)$. The statistics of primordial metric fluctuations are encoded equally in any cosmological observable and thus is only sensitive to the number of observed (quasi-linear) modes.  In contrast, the physics of structure formation itself depends on the specific probe, as the transfer functions are sensitive to the forces that act on each individual particle.  

In addition, direct measurements relic gravitational waves are not only proportional to the gravitational waves generated during inflation, but also new sources of gravitational waves generated during reheating or later.  


Cosmic surveys probe the universe at a variety of redshifts.  High redshifts are more sensitive to the physics of the radiation era and are generally more linear.  Lower redshift probes are more sensitive to the matter contend of the universe but also the nonlinear evolution that controls the formation of structure.  For this reason, cosmic surveys are largely complementary.  On the other hand, for tests of inflation, where the number of modes is the primary factor, three-dimensional surveys can carry vastly more information, if the problem of nonlinear evolution could be circumvented.

\subsection{Epochs}

\subsubsection{$z\sim1000$}


\subsubsection{$150 \gtrsim z \gtrsim 20$: Dark Ages}
The Dark Ages are of tremendous cosmological interest. The epoch provides access to a huge number of Fourier modes of the matter density fields \citep{Loeb2004}. They are a particularly clean probe of the matter field since this is prior to the formation of the first luminous sources, thus obviating the need for the modelling of complicated astrophysics. The theoretical modelling effort is in fact even simpler than, say, that needed for galaxy surveys, since at these high redshifts, matter fluctuations are in the linear perturbative regime even at very fine scales. This is important because the spatial fluctuations exist to extremely small scales, as they are not Silk damped and therefore persist down to the Jeans scale \citep{Tegmark2009}. The result is a vast number of modes that can be in principle be used to probe fundamental cosmology. The long lever arm in scale, from the largest structures to the smallest structures, enables constraints on the running of the matter power spectrum's spectral index \citep{Mao2008}. This would represent an incisive probe of the inflationary paradigm. Future measurements may also be able to detect features in the primordial power spectrum \citep{Chen2016Features}, or to detect primordial non-Gaussianity~\citep{Munoz2015nonGaussianity}. In addition, the 21\,cm line can be used to probe the existence of relic gravitational waves from inflation, either through their direct effects on large scale structure \citep{Masui2010} or through their lensing effects \citep{Book2012}. Tests of statistical isotropy and homogeneity may also be possible \citep{Shiraishi2016}. Small-scale measurements enable measurements of the neutrino mass \citep{Mao2008} and constraints on the existence of warm dark matter \citep{Loeb2004}. Finally, the cleanliness of measurements during the Dark Ages provide a good platform for detecting exotic phenomena beyond the standard models of particle physics and cosmology (see references in \cite{Furlanetto2019fundamentalphysics}).

\subsubsection{$20 \gtrsim z \gtrsim 5.5$: Cosmic Dawn and Reionization}
As the first luminous objects begin to form, the 21\,cm line ceases to directly trace the dark matter distribution. Radiation from these objects affects the spin temperature and ionization state of the intergalactic medium (IGM) in a spatially and temporally non-trivial way. This is reflected in the spatial fluctuations and redshift evolution of the 21\,cm line, which is no longer governed by the relatively simple physics of cosmological matter perturbations alone. This is both a defect and an opportunity. It is an opportunity because it provides a promising tool for understanding the nature of the first luminous objects. It is a defect because the complicated astrophysics of the era means that one must be more creative in extracting information about fundamental physics. However, several promising avenues have emerged in recent years on this front. For example, velocity-induced acoustic oscillations \citep{Dalal2010,Fialkov2012VAOs,Munoz2019VAOs1,McQuinn2012VAOs} have the potential to serve as clean standard rulers at high redshifts---even in the presence of the astrophysics of Cosmic Dawn---thus enabling precision measurements of the Hubble expansion rate \citep{Munoz2019VAOs2}. It may also be possible to parameterize (and marginalize out) any messy astrophysics in a fairly model-agnostic way using effective field theory techniques \cite{McQuinn:2018, Hoffmann:2019,2022arXiv220506270Q}. Machine-learning techniques may also allow the ``undoing" of some astrophysical effects \cite{2021ApJ...907...44V}. Probes of small-scale cosmological structure through their couplings to large scales have shown promising signs of being relatively robust to changes in astrophysical modelling \cite{2020PhRvD.101f3526M}. Finally, combinations of 21\,cm measurements with CMB measurements can provide complementary constraints that remove reionization as a nuisance for CMB measurements \cite{2021arXiv211206933B,Sailer:2022vqx}, sharpening constraints on fundamental primordial physics \cite{Liu:2016,Billings:2021,Fialkov:2016}. Taken together, this suggests a path forward to leveraging the large number of (linear) Fourier modes and their large dynamic range in lengthscale, even in the Cosmic Dawn and Reionization era. The challenges here are data interpretation and the more sophisticated analyses needed to get around the astrophysics; this is thus complementary to futuristic Dark Ages efforts, which are easier to interpret but are technically harder measurements from an instrumental standpoint.

\subsubsection{$z\lesssim 5$: post-reionization}
Observations within this epoch are mapping the large-scale structure of the Universe, giving them the ability to do much of the same science as optical galaxy redshift surveys. However, as they can naturally have wide fields of view and observe all redshifts in their band simultaneously, IM experiments are more readily able to quickly survey very large volumes than optical galaxy redshift surveys. And as they do not need to resolve individual galaxies, they can more easily push to high redshifts, through the redshift desert ($z\sim 1$--$3$, where optical spectroscopy is challenging) and beyond ($3 \lesssim z \lesssim 6$).

As IM is a very recent technique that is still being developed, the initial target within this era are to measure Baryon Acoustic Oscillations (BAO). These are the remnants of primordial sound waves that leave a distinct signature in the correlation structure of matter, and they can be used as a standard ruler, albeit a statistical one, to measure the expansion history of the Universe \citep{1998ApJ...504L..57E,Seo2003}. The BAO signature is quite distinct and thus more robust to systematics, making it an ideal first science target for 21\,cm IM experiments. As a bonus, one can push to ranges in redshifts not currently probed by existing optical surveys \citep{Peterson:2006,Chang2008,2008MNRAS.383.1195W}. By constraining the expansion history of our Universe we hope to be able to infer the properties of Dark Energy, in particular its equation of state $w(z)$, which can yield clues to a microphysical explanation. Such constraints on the equation of state could potentially shed light on recent tensions in measurements of the Hubble parameter \citep{Knox2019HubbleHunter}, particularly in the context of proposed explanations that have non-trivial time evolution of dark energy at $z \gtrsim 1$ (e.g., \cite{DiValentino2016,DiValentino2017,Keeley2019}).

As IM is able to survey very large volumes of the Universe with precise radial distances (unlike photometric redshift surveys) it is ideal for discovering small statistical effects where measuring a large number of modes is essential. One target is looking for features in the power spectrum which might tell us about inflationary physics \citep{Chluba2018, Slosar:2019gvt}. Another is looking for signatures of new physics by searching for non-Gaussianity in 21\,cm data \citep{2017PhRvD..96f3525L, Meerburg:2019qqi}.

The expansion history information that IM can obtain from BAO, combined with broadband measurements of the power spectrum shape, plus future Cosmic Microwave Background measurements gives a potent combination for probing the contents of the Universe. In particular the number of relativistic degrees of freedom and the sum of the neutrino masses \citep{2016JCAP...02..008O,2018JCAP...05..004O} can be constrained to $\lesssim 20\,{\rm meV}$ by combining IM with other probes.

On extremely large scales there are general relativistic corrections to the standard observables \citep{2011PhRvD..84d3516C}, that if observed could be a stringent confirmation of the current cosmological model. To measure these, one needs to map large volumes of the Universe to build up enough samples of these scales (for which IM is ideally suited), and to combine with other probes on similar scales (e.g., photometric surveys like the Large Synoptic Survey Telescope) in order to remove sample variance effects \citep{2015PhRvD..92f3525A}.

Although one only directly measures the inhomogeneity in the distribution of HI with 21\,cm IM, by looking at the distortions in the observed three-dimensional field caused by gravitational lensing, one can in principle infer the \emph{total matter} distribution within the volume \citep{Foreman2018}. As the lensing displacements are typically small, upcoming 21\,cm experiments may only be able to see this effect in cross correlation with photometric redshift surveys, but it will be extremely powerful for following generations of instruments.



==> old tex/Primordial_GW.tex <==
\section{Primordial Gravitational Waves \textcolor{red}{dan, vuk, deirdre 5 pages}}
\label{sec:pGW}

\begin{figure}[!t]
\begin{center}
\includegraphics[width=1\hsize]{Figures/landscape_Snowmass2022_CF5fig1.png}
\end{center}
\caption{Landscape of gravitational wave cosmology. Experimental results include: O1-O3 LIGO-Virgo upper limits~\cite{PhysRevD.104.022004}, indirect limits from big bang nucleosynthesis~\cite{PhysRevX.6.011035}, CMB limits~\cite{PhysRevX.6.011035}, and Parkes pulsar timing limit~\cite{PhysRevX.6.011035}, as well as projected sensitivities of the third generation (3G) terrestrial GW detectors~\cite{EinsteinTelescope,CosmicExplorer} and LISA~\cite{LISA}. Theoretical models include examples of slow-roll inflation~\cite{turner}, Axion Inflation~\cite{peloso_parviol}, hypothetical stiff equation of state in the early universe~\cite{boylebuonanno}, and foregrounds due to binary black hole/neutron stars~\cite{PhysRevD.104.022004} and galactic binary white dwarfs~\cite{LISA}.
}
\label{fig:landscape_inflation}
\end{figure}

In the standard inflationary paradigm, vacuum fluctuations of the inflaton field may lead to a scale-invariant spectrum of \gw{s}. These vacuum fluctuations are imprinted onto the Cosmic Microwave Background (CMB) in the form of B-mode polarization. They are also amplified as the universe transitions into the radiation-dominated phase (and again later, when it transitions into the matter-dominated phase), resulting in a nearly frequency-independent \gw{} energy density spectrum $\Omega_{\rm GW}(f)$ (normalized by the critical energy density of the universe). The energy density spectrum of the stochastic gravitational wave background (SGWB) in this standard inflationary model is depicted in Fig. \ref{fig:landscape_inflation}, in comparison with other possible SGWB models and experimental results and sensitivities. \comment{Deirdre: I think this previous sentence is unclear.  It is a plot of SGWB or is it a plot comparing SGWB models? - Vuk: I modified the sentence, hopefully it is clearer?}

\comment{Deirdre: Could we introduce the ratio of the power spectra of the tensor and scalar modes measures blah blah so readers see its usefulness immediately?}
Inflationary models generally predict very small values of the ratio of the power spectra of the tensor and scalar modes $(r\ll 1)$. This also implies relatively weak SGWB spectrum $\Omega_{\rm GW}(f)$---as shown in Fig. \ref{fig:landscape_inflation}; and, therefore, this background will likely be out of reach of the planned next-generation \gw{} detectors. However, a number of other processes during and/or after inflation could lead to significantly stronger SGWB that may be detectable by upcoming experiments. As an example, inflationary scenarios in which the inflaton couples to a gauge field may predict strongly blue-tilted \gw{} spectra that may be consistent with CMB bounds at long wavelengths but within reach of direct detection experiments at short wavelengths. (See Ref.~\cite{Thorne:2017jft} for examples, or the forthcoming ``Cosmology with the Laser Interferometer Space Antenna,'' by the LISA Cosmology Working Group \cite{Auclair:2022lcg}, for further discussion.)

\subsection{Alternatives to Inflation}

Despite its success, inflation does face drawbacks \cite{Goldwirth:1989pr,Calzetta:1992gv,Calzetta:1992bp,Borde:2001nh,Ijjas:2014nta,Brandenberger:2000as} and various alternatives have been proposed: examples include the pre-Big Bang \cite{Gasperini:1992em} model, the ekpyrotic model \cite{Khoury:2001wf}, the string gas cosmology \cite{Brandenberger:1988aj,Battefeld:2014uga},
 and the matter bounce scenario \cite{Finelli:2001sr,Brandenberger:2012zb}. 

The pre-Big Bang scenario \cite{Gasperini:1992em,Gasperini:2002bn} assumes that
gravity and cosmology are based on some particular version of superstring theory. According to this model, the Universe  emerges from a highly perturbative initial state preceding the Big Bang. 
In string theory, the dilaton is an additional massless mode, which while at late times may be assumed fixed, is dynamical in the very early Universe. Hence, the massless sector of string theory to which the graviton belongs is given by dilaton gravity. 
This model leads to the production of an amplified quasi-thermal spectrum of gravitons during the dilaton-driven phase. While the slope of the \gw{} spectrum may change for modes crossing the horizon during the subsequent string phase, it remains characterized by an enhanced production of high frequency gravitons, irrespective of the particular value of the spectral index \cite{Brustein:1995ah}. For a wide region of the parameter space of the pre-Big Bang model, one can simultaneously generate a spectrum of scalar metric perturbations in agreement with Planck data and a stochastic background of primordial \gw{s} within reach of the design sensitivity of aLIGO/Virgo and/or LISA \cite{Gasperini:2016gre}.

The ekpyrotic model \cite{Khoury:2001wf} is motivated by a specific realization of M-theory in which spacetime is 11-dimensional \cite{Horava:1995qa}. In this model, whereas the equation of motion of the cosmological perturbations depends on the potential of the scalar field, that of the \gw{s} does not. The spectrum of \gw{s} turns out to be very blue, implying that primordial \gw{s} are negligible on scales of cosmological interest today. 

String gas cosmology is based on degrees of freedom and symmetries of superstring theory which are absent in an effective
field theory approach to early Universe cosmology.
This model has two fundamental elements. The first is the Hagedorn temperature defined as  the maximal temperature which a gas
of strings in thermal equilibrium can achieve. The second is the T-duality symmetry of the spectrum of string states.
This string gas cosmology model (tested also via numerical experiments \cite{Sakellariadou:1995vk})  leads to an almost scale-invariant spectrum of primordial \gw{s} \cite{Brandenberger:2006vv}. However, whereas inflation typically leads to a red spectrum, string gas cosmology generically yields a slightly blue spectrum.  

The matter bounce model \cite{Finelli:2001sr,Brandenberger:2012zb}  is based on the duality between the evolution of the canonical fluctuation variables in an exponentially expanding period and in a contracting phase with vanishing pressure. In this model, the amplitude of the GW spectrum is generically larger than that in  inflationary models ($r$ can be close to 1).

\subsection{Inflation and the Subsequent Phases}

Having indicated the many possibilities during the expansion phase in the very early Universe, we now turn to the role that \gw{s} play in the subsequent eras. 
While the CMB limits the scale of inflation to be smaller than $\mathcal{O}(10^{16})$ GeV, the Big Bang Nucleosynthesis (BBN) constraints imply that the universe was radiation dominated when neutrinos decoupled from the primordial plasma, around $\mathcal{O}(1)$ MeV. The vast stretch of energies between these two energy scales could host a variety of cosmological histories and fundamental particle processes. \gw{s}, because they free-stream through the entirety of cosmological history, provide a way of probing the cosmic history before BBN. In this sense, the SGWB serves as a \textit{cosmic witness} that records information about the fundamental particle physics processes that took place in the pre-BBN era, at energies far above those accessible in accelerators.


$(i)$ Long-lasting \gw{} sources as cosmic witnesses: The vast stretch of energies between the initial expansion phase of the Universe and BBN can accommodate a range of non-standard cosmological histories with equations of state parameter $w$ different from $w=1/3$. The \gw{} spectrum of long-lasting sources such as inflation and  networks of cosmic strings spans a wide range of frequencies and has been studied  as cosmic witnesses \cite{DEramo:2019tit, Figueroa:2019paj}, especially to extract information about $w$.  Scenarios with $1/3 \leq w \leq 1$ %corresponds to scenarios with a stiff fluid dominating the epoch between the end of inflation and the onset of radiation domination. These scenarios 
develop a blue tilt for the tensor perturbations at large frequencies and certain portions of the parameter space may be detectable by LISA and/or terrestrial \gw{} detectors \cite{boylebuonanno,Figueroa:2019paj,Giovannini_1,Giovannini_2}, c.f. Fig. \ref{fig:landscape_inflation}.   Matter-dominated era with $w=0$ may cause kinks in the spectrum at frequencies corresponding to the onset of matter and radiation domination, which may be observable in the future at BBO and other experiments. 
If the  change in the equation of state is sudden enough, rapidly oscillating scalar perturbations may enhance the primordial \gw{} spectrum from inflation; this effect has been pursued in the context of primordial black holes \cite{Inomata:2020lmk} and Q-balls \cite{White:2021hwi}.









$(ii)$ Phase transitions as cosmic witnesses: It is challenging to use shorter-lasting sources like phase transitions as a witness to  $w$ in the early universe, although some effort has been made in this direction \cite{Guo:2020grp, Hook:2020phx, Barenboim:2016mjm, Cai:2019cdl}. 

If the phase transition occurs during a phase dominated by an entity with a general equation of state $w$ that is not radiation, expressions for the parameters defining the phase transition should take into account the new dominant contribution to the energy density; if the phase transition is followed by an era dominated by an entity with state $w$, the modified redshifting changes the spectrum. In the deep infrared, super-horizon modes scale as $\propto k^{3+2\frac{3w-1}{3w+1}}$. 
A special case of phase transitions serving as a probe of inflationary physics is when the transition occurs \textit{during} inflation itself, possibly triggered by inflaton couplings to spectator fields. For such a source, the \gw{} spectrum always contains a unique oscillatory feature, which can be used to identify the \gw{} source~\cite{An:2020fff}.

A different avenue is to use \gw{s} from phase transitions as a record of temperature anisotropies coming from a previous era, for example from inflation. Since the phase transition inherits primordial temperature anisotropies, it effectively serves as a copy of the CMB, but in an earlier, more pristine form \cite{Geller:2018mwu}. While this matching  is true for  adiabatic fluctuations, if the primordial fluctuations  carry an  isocurvature component then a richer scenario can emerge \cite{Kumar:2021ffi}. 


$(iii)$ \gw{s} from inflationary reheating/preheating: The large  time-dependent field inhomogeneities that are characteristic of rapid particle production through parametric resonances during a preheating phase \cite{Kofman:1997yn, Kofman:1994rk, Amin:2014eta} can be a well-motivated source of \gw{} production. Topics that have been explored in this context include  gauge preheating after axion inflation  \cite{Adshead:2019lbr, Adshead:2018doq}, self-resonance after single-field inflation and oscillon formation \cite{Zhou:2013tsa,Lozanov:2019ylm, Antusch:2016con, Amin:2018xfe, Hiramatsu:2020obh,Kou:2021bij}, as well as tachyonic preheating from a waterfall transition \cite{Garcia-Bellido:2007nns, Garcia-Bellido:2007fiu, Dufaux:2010cf}. The frequency of the resultant \gw{} signal is typically too high, or the amplitude too small, to be detectable with near future \gw{} detectors, although several ideas have been proposed recently \cite{Berlin:2021txa, Domcke:2022rgu}.  The recent work of  \cite{Cui:2021are} demonstrates a promising \gw{} detection prospect based on a preheating scenario in the framework of hybrid inflation, where a prolonged waterfall phase allows for an efficient transfer of energy from the scalar sector to an Abelian gauge field.
For particular reheating mechanisms, the study of \cite{Haque:2021dha} has investigated the phases of early and late time reheating through imprints on primordial \gw{s}.





==> old tex/Primordial_Structure.tex <==
\section{Primordial Structure, \textcolor{red}{dan, adrian, laura 5 pages}}
\label{sec:pStruc}

Structure in the universe is believed to have originated during inflation from quantum fluctuations of the inflaton or, equivalently, the scalar mode of the metric. These fluctuations change the amount of inflation that occured in different parts of the universe, and thus correspond to a change in the physical energy densities from place to place.  After reheating, these density perturbations grow and evolve as the re-enter the cosmic horizon.  The different components of the energy density and their fundamental interactions shape this subsequent evolution, giving rise (at linear order) t
\beq
\delta_{i}(\vec k,z) = T_i(k,z) \zeta(\vec k)
\eeq
where $\vec k$ is a comoving wave-number, $k= |\vec k|$, $\zeta(\vec k)$ is the scalar metric fluctuation, $\delta(\vec k,i)$ is the density contrast of species $i$ and $T_i(k,i)$ is its transfer function.  

Measurements of the statistical properties of these densities encode both the physics of inflation and of the evolution of the universe after the hot-bang bang.  For example, the total matter power spectrum, 
\beq
P_{m}(k,z) = T^2_m(k,z) P_\zeta(k) \ ,
\eeq
is both a measurement of the power spectrum from inflation, $P_\zeta(k)$, and the growth of structure, BAO, etc. through the transfer function $T_m(k,z)$. The statistics of primordial metric fluctuations are encoded equally in any cosmological observable and thus is only sensitive to the number of observed (quasi-linear) modes.  In contrast, the physics of structure formation itself depends on the specific probe, as the transfer functions are sensitive to the forces that act on each individual particle.  

Cosmic surveys probe the universe at a variety of redshifts.  High redshifts are more sensitive to the physics of the radiation era and are generally more linear.  Lower redshift probes are more sensitive to the matter contend of the universe but also the nonlinear evolution that controls the formation of structure.  For this reason, cosmic surveys are largely complementary.  On the other hand, for tests of inflation, where the number of modes is the primary factor, three-dimensional surveys can carry vastly more information, if the problem of nonlinear evolution could be circumvented.

\subsubsection{Inflation}

Inflation is defined by two fundamental properties. First, it is a period of of nearly exponential expansion, such that the expansion rate $H(t) = \dot a/a$ is nearly constant, $|\dot H| \ll H^2$. Second, inflation includes a physical degree of freedom that behaves a clock, effectively telling the universe when to end inflation.  Like any clock, it is subject to errors from quantum fluctuations giving rise to the density fluctuations.

The physics of inflation is characterized by energy scales that are relevant for various physical processes, illustrated in Figure~\ref{fig:inflation}. In practice, what we observe are dimensionless rations involved the Hubble scale during inflation, $H$, and these other physical scales.  Measurements to date determine the scale of the background evolution $f$, which in the case of conventional slow roll inflation is given by speed of the background scalar field, $f^2 = |\dot \phi$.  The spectral tilt, $n_s$, encodes the time evolution of inflationary parameters such as $\dot H / H^2 \ll 1$.  

\begin{figure}[h!]
\centering
\includegraphics[width=3.5in]{Figures/inflation.pdf}
\caption{Energy scales relevant to inflation. Reproduced from~\cite{Achucarro:2022qrl}. }
\label{fig:inflation}
\end{figure}

Future probes of inflation can be roughly characterized by three new scales that are parameterized by the variables, $A_{\rm lin}$, $f_{\rm NL}$ and $A_t$.  The first parameter,  $A_{\rm lin}$, is a characteristic scale of features in the inflationary power spectrum (and/or higher point correlators). This is a signal of the breaking of scale invariance, which indicates that there is a characteristic time-scale associated with inflation beyond $f$. The precise form of the features encodes the physics responsible.  

The second, $\fnl$, is the amplitude of primordial non-Gaussianity.  The third, $A_t$, is the amplitude of primordial gravitational waves and is typically fixed in terms of $H$ in terms of the Planck scale, $M_{\rm pl}$.  

\subsubsection{$z\sim1000$}
(Grab from CMBS4 white paper)

\subsubsection{$z\sim20$}
The Dark Ages are of tremendous cosmological interest. The epoch provides access to a huge number of Fourier modes of the matter density fields \citep{Loeb2004}. They are a particularly clean probe of the matter field since this is prior to the formation of the first luminous sources, thus obviating the need for the modelling of complicated astrophysics. The theoretical modelling effort is in fact even simpler than, say, that needed for galaxy surveys, since at these high redshifts, matter fluctuations are in the linear perturbative regime even at very fine scales. This is important because the spatial fluctuations exist to extremely small scales, as they are not Silk damped and therefore persist down to the Jeans scale \citep{Tegmark2009}. The result is a vast number of modes that can be in principle be used to probe fundamental cosmology. The long lever arm in scale, from the largest structures to the smallest structures, enables constraints on the running of the matter power spectrum's spectral index \citep{Mao2008}. This would represent an incisive probe of the inflationary paradigm. Future measurements may also be able to detect features in the primordial power spectrum \citep{Chen2016Features}, or to detect primordial non-Gaussianity~\citep{Munoz2015nonGaussianity}. In addition, the 21\,cm line can be used to probe the existence of relic gravitational waves from inflation, either through their direct effects on large scale structure \citep{Masui2010} or through their lensing effects \citep{Book2012}. Tests of statistical isotropy and homogeneity may also be possible \citep{Shiraishi2016}. Small-scale measurements enable measurements of the neutrino mass \citep{Mao2008} and constraints on the existence of warm dark matter \citep{Loeb2004}. Finally, the cleanliness of measurements during the Dark Ages provide a good platform for detecting exotic phenomena beyond the standard models of particle physics and cosmology (see references in \cite{Furlanetto2019fundamentalphysics}).

\subsubsection{$z\sim10$}
As the first luminous objects begin to form, the 21\,cm line ceases to directly trace the dark matter distribution. Radiation from these objects affects the spin temperature and ionization state of the intergalactic medium (IGM) in a spatially and temporally non-trivial way. This is reflected in the spatial fluctuations and redshift evolution of the 21\,cm line, which is no longer governed by the relatively simple physics of cosmological matter perturbations alone. This is both a defect and an opportunity. It is an opportunity because it provides a promising tool for understanding the nature of the first luminous objects. It is a defect because the complicated astrophysics of the era means that one must be more creative in extracting information about fundamental physics. However, several promising avenues have emerged in recent years on this front. For example, velocity-induced acoustic oscillations \citep{Dalal2010,Fialkov2012VAOs,Munoz2019VAOs1,McQuinn2012VAOs} have the potential to serve as clean standard rulers at high redshifts, thus enabling precision measurements of the Hubble expansion rate \citep{Munoz2019VAOs2}. It may also be possible to parametrize (and marginalize out) any messy astrophysics in a fairly model-agnostic way using effective field theory techniques \cite{McQuinn:2018, Hoffmann:2019}. Machine-learning techniques may also allow the ``undoing" of some astrophysical effects \cite{2021ApJ...907...44V}. Probes of small-scale cosmological structure through their couplings to large scales have shown promising signs of being relatively robust to changes in astrophysical modelling \cite{2020PhRvD.101f3526M}. Finally, combinations of 21\,cm measurements with CMB measurements can provide complementary constraints that remove reionization as a nuisance for CMB measurements \cite{2021arXiv211206933B}, sharpening constraints on fundamental physics \cite{Liu:2016,Billings:2021,Fialkov:2016}.
% Expand on VAOs from a sort of 1 sentence level to about 3 sentence level
% Things should be in service of inflation. E.g., tau breaking degeneracies

\subsubsection{$z\sim5$}
Observations within this epoch are mapping the large-scale structure of the Universe, giving them the ability to do much of the same science as optical galaxy redshift surveys. However, as they can naturally have wide fields of view and observe all redshifts in their band simultaneously, IM experiments are more readily able to quickly survey very large volumes than optical galaxy redshift surveys. And as they do not need to resolve individual galaxies, they can more easily push to high redshifts, through the redshift desert ($z\sim 1$--$3$, where optical spectroscopy is challenging) and beyond ($3 \lesssim z \lesssim 6$).

As IM is a very recent technique that is still being developed, the initial target within this era are to measure Baryon Acoustic Oscillations (BAO). These are the remnants of primordial sound waves that leave a distinct signature in the correlation structure of matter, and they can be used as a standard ruler, albeit a statistical one, to measure the expansion history of the Universe \citep{1998ApJ...504L..57E,Seo2003}. The BAO signature is quite distinct and thus more robust to systematics, making it an ideal first science target for 21\,cm IM experiments. As a bonus, one can push to ranges in redshifts not currently probed by existing optical surveys \citep{Peterson:2006,Chang2008,2008MNRAS.383.1195W}. By constraining the expansion history of our Universe we hope to be able to infer the properties of Dark Energy, in particular its equation of state $w(z)$, which can yield clues to a microphysical explanation. Such constraints on the equation of state could potentially shed light on recent tensions in measurements of the Hubble parameter \citep{Knox2019HubbleHunter}, particularly in the context of proposed explanations that have non-trivial time evolution of dark energy at $z \gtrsim 1$ (e.g., \cite{DiValentino2016,DiValentino2017,Keeley2019}).

As IM is able to survey very large volumes of the Universe with precise radial distances (unlike photometric redshift surveys) it is ideal for discovering small statistical effects where measuring a large number of modes is essential. One target is looking for features in the power spectrum which might tell us about inflationary physics \citep{Chluba2018, Slosar:2019gvt}. Another is looking for signatures of new physics by searching for non-Gaussianity in 21\,cm data \citep{2017PhRvD..96f3525L, Meerburg:2019qqi}.

The expansion history information that IM can obtain from BAO, combined with broadband measurements of the power spectrum shape, plus future Cosmic Microwave Background measurements gives a potent combination for probing the contents of the Universe. In particular the number of relativistic degrees of freedom and the sum of the neutrino masses \citep{2016JCAP...02..008O,2018JCAP...05..004O} can be constrained to $\lesssim 20\,{\rm meV}$ by combining IM with other probes.

On extremely large scales there are general relativistic corrections to the standard observables \citep{2011PhRvD..84d3516C}, that if observed could be a stringent confirmation of the current cosmological model. To measure these, one needs to map large volumes of the Universe to build up enough samples of these scales (for which IM is ideally suited), and to combine with other probes on similar scales (e.g., photometric surveys like the Large Synoptic Survey Telescope) in order to remove sample variance effects \citep{2015PhRvD..92f3525A}.

Although one only directly measures the inhomogeneity in the distribution of HI with 21\,cm IM, by looking at the distortions in the observed three-dimensional field caused by gravitational lensing, one can in principle infer the \emph{total matter} distribution within the volume \citep{Foreman2018}. As the lensing displacements are typically small, upcoming 21\,cm experiments may only be able to see this effect in cross correlation with photometric redshift surveys, but it will be extremely powerful for following generations of instruments.



==> old tex/Rel_Energy.tex <==
% DO NOT USE THIS SECTION - GO TO RELICS

\section{Relativistic Energy in the Early Universe \textcolor{red}{Renee, Vuk, 5 pages}}
\label{sec:RE}
\begin{figure}[!t]
\begin{center}
\includegraphics[width=1\hsize]{Figures/landscape_Snowmass2022_CF5fig2.png}
\end{center}
\caption{Same as Fig. \ref{fig:landscape_inflation}, but focused on models of phase transitions and topological defects. Theoretical models include examples of first-order phase transitions (PT-1~\cite{Ellis:2019oqb}, PT-2~\cite{DelleRose:2019pgi}, and PT-3~\cite{An:2022}), cosmic strings~\cite{Siemens:2006yp}, and foregrounds due to binary black hole/neutron stars~\cite{PhysRevD.104.022004} and galactic binary white dwarfs~\cite{LISA}.
}
\label{fig:landscape_PT}
\end{figure}


\subsection{Phase Transitions}

GWs from first order phase transitions (FOPTs) in the early Universe offer a unique way of probing particle physics models at energy scales otherwise inaccessible. Such phase transitions could occur at nearly any time during or after inflation. The GW spectrum, with examples shown in Fig.~\ref{fig:sample}, is sensitive to the shape of the effective potential, which depends on the symmetry breaking pattern and the particle content of the theory. This provides access to regions of parameter
space unexplored so far in various extensions of the SM. GWs from a strong FOPT have a plethora of motivations in the early universe. For instance, new states at the electroweak scale can catalyze a strongly first order electroweak phase transition \cite{Ramsey-Musolf:2019lsf,Profumo:2007wc,Delaunay:2007wb,Huang:2016cjm,Chala:2018ari,Croon:2020cgk,Grojean:2006bp,Alves:2018jsw,Alves:2020bpi,Vaskonen:2016yiu,Dorsch:2016nrg,Chao:2017vrq,Wang:2019pet,Demidov:2017lzf,Ahriche:2018rao,Huang:2017rzf,Mohamadnejad:2019vzg,Baldes:2018nel,Huang:2018aja,Ellis:2019flb, Alves:2018oct, Alves:2019igs,Cline:2021iff,Chao:2021xqv,Liu:2021mhn,Zhang:2021alu,Cai:2022bcf} and large lepton asymmetries or different  quark masses can make the QCD transition strong \cite{Schwarz:2009ii,Middeldorf-Wygas:2020glx,Caprini:2010xv,vonHarling:2017yew}. Beyond this, a strong transition can occur in multistep phase transitions\footnote{See Refs. \cite{Weinberg:1974hy,Land:1992sm,Patel:2012pi,Patel:2013zla,Blinov:2015sna} for the viability of a multistep phase transition} \cite{Niemi:2018asa,Croon:2018new,Morais:2018uou,Morais:2019fnm,Angelescu:2018dkk,TripletGW2022}, B-L breaking \cite{Jinno:2016knw,Chao:2017ilw,Brdar:2018num,Okada:2018xdh,Marzo:2018nov,Bian:2019szo,Hasegawa:2019amx,Ellis:2019oqb,Okada:2020vvb} (or B/L breaking \cite{Fornal:2020esl}), flavour physics \cite{Greljo:2019xan,Fornal:2020ngq}, axions \cite{Dev:2019njv,VonHarling:2019rgb,DelleRose:2019pgi}, GUT symmetry breaking chains \cite{Hashino:2018zsi,Huang:2017laj,Croon:2018kqn,Brdar:2019fur,Huang:2020bbe}, supersymmetry breaking \cite{Fornal:2021ovz,Craig:2020jfv,Apreda:2001us,Bian:2017wfv}, hidden sector involving scalars \cite{Schwaller:2015tja,Baldes:2018emh,Breitbach:2018ddu,Croon:2018erz,Hall:2019ank,Baldes:2017rcu,Croon:2019rqu,Hall:2019rld,Hall:2019ank,Chao:2020adk,Dent:2022bcd}, neutrino mass models \cite{Li:2020eun,DiBari:2021dri,Zhou:2022mlz} and confinement \cite{Helmboldt:2019pan,Aoki:2019mlt,Helmboldt:2019pan,Croon:2019ugf,Croon:2019iuh,Garcia-Bellido:2021zgu,Huang:2020crf,Halverson:2020xpg,Kang:2021epo}.

In thermal phase transitions, bubbles of the new vacuum expand in a plasma of ultrarelativistic particles. Interactions of the particles with the bubble walls determine the terminal wall velocity $v_w$ of the bubbles. GWs are generated in collisions of bubble walls \cite{Kosowsky:1991ua,Kosowsky:1992vn,Huber:2008hg,Jinno:2016vai}, as well as in the fluid shock configurations, detonation or deflagrations, accompanying them \cite{Kamionkowski:1993fg}.
After the bubbles have merged, a bulk fluid velocity will remain in the plasma. 
The velocity perturbations will typically be longitudinal, unless the bubbles have been deformed during the transition due to hydrodynamic instabilities or deformations of the shape. 
In weak transitions, the fluid perturbation will take the form of longitudinal acoustic waves -- sound waves 
\cite{Hindmarsh:2013xza}. 
Shocks will form, typically in strong transitions leading to turbulence \cite{Pen:2015qta}, if the shock formation timescale $\tau_\text{sh} \sim L_*/v_\text{rms}$, where $L_*$ is a typical length scale in the fluid linked to the mean bubble separation, 
and $v_\text{rms}$ is the root mean square fluid 3-velocity, is smaller than the Hubble time \cite{Caprini:2015zlo}. 
Sound waves, acoustic, and vortical turbulence are all sources of GWs, lasting until the kinetic energy is dissipated by the plasma viscosity \cite{Caprini:2009yp}.
These different processes source GWs with different spectral shapes (see e.g.~\cite{Hindmarsh:2017gnf,Hindmarsh:2019phv,Niksa:2018ofa,Caprini:2009yp,RoperPol:2019wvy,Jinno:2020eqg}), as illustrated in Fig. \ref{}, allowing the possibility of reconstructing the conditions during and after the FOPT.

Theoretical and numerical modelling of phase transitions is a very active area. 
Four parameters are critical for determining the GW production: the nucleation temperature $T_*$, the bubble wall velocity $v_w$, the FOPT's strength $\alpha$ and its inverse duration $\beta$. Multiple open questions are under investigation focused on estimating these parameters.
First, a perturbative treatment of the finite temperature potential is known to breakdown. The central problem is that the expansion parameter at finite temperature involves a mode occupation
which diverges when the mass vanishes \cite{Linde:1980ts}. Currently, only the technique of dimensional reduction \cite{Kajantie:1995dw,Farakos:1994xh} performed at NLO using an $\hbar$ expansion provides a prescription to calculate thermodynamic parameters at $O(g^4)$ in a gauge independent way \cite{Croon:2020cgk,Gould:2021oba}. This method is challenging to use and has been applied to benchmarks in very few models. Proposed alternatives to dimensional reduction \cite{Curtin:2016urg,Croon:2021vtc} are in need of further development and testing. Second, an accurate evaluation of the nucleation rate $\Gamma_{\mathrm{nuc}}$ and its evolution with temperature is critical for defining the characteristic time scales of the transition. 
For sufficiently fast transitions, $T_{\ast}$ and $\beta$ can be obtained by linearizing the rate  near $T_{\ast}$. This breaks down for slow transitions, which can be of great phenomenological interest, where the next order corrections must be accounted for~\cite{Ellis:2018mja}. A number of other issues that affect the nucleation rate also require further study \cite{GW_EarlyUniv_WP}. 
Third, the bubble wall speed can be calculated via different formalisms whose applicability depends on the relative strengths of the transition that determine
whether the terminal speed will be only mildly relativistic or ultrarelativistic. This is also investigated by many authors~\cite{Konstandin:2010dm,BarrosoMancha:2020fay,Balaji:2020yrx,Ai:2021kak,Cline:2021iff,Bodeker:2009qy,Bodeker:2017cim,Hoeche:2020rsg,Gouttenoire:2021kjv,GW_EarlyUniv_WP}.

In non-thermal transitions, the vacuum energy released in phase transitions can far exceed the surrounding radiation energy ~\cite{Randall:2006py,Espinosa:2008kw}.
Here the bubble expansion mode has two possibilities~\cite{Espinosa:2010hh}: (i) strong detonation, where the wall reaches a terminal velocity due to balancing between the outward pressure and the friction, and GW production comes from a highly relativistic and concentrated fluid around the bubbles, and (ii) a runaway, where the wall continues to accelerate until it collides producing GWs~\cite{Ellis:2019oqb}. Both scenarios are being investigated, e.g. through the bulk flow runaway model~\cite{Jinno:2017fby,Konstandin:2017sat,Megevand:2021juo}, and the sound shell detonation model~\cite{Hindmarsh:2016lnk,Hindmarsh:2019phv}.

In addition, both purely hydrodynamic and magneto-hydrodynamic (MHD) turbulence are expected to source GWs \cite{Kamionkowski:1993fg}.
Past analyses have evaluated the GW production using semi-analytical modelling \cite{Kosowsky:2001xp,Dolgov:2002ra,Caprini:2006jb,Gogoberidze:2007an,Kahniashvili:2008pe,Caprini:2009yp,Niksa:2018ofa}. Simulation-based approaches are also being pursued \cite{Cutting:2019zws,RoperPol:2019wvy,Kahniashvili:2020jgm,RoperPol:2021xnd,RoperPol:2022iel}. 

\subsubsection{Complementarity with Collider-Based Searches}

Unravelling the physics behind the electroweak symmetry breaking (EWSB) is a leading target of the upcoming LHC and HL-LHC physics runs, as well as a main physics driver for future high-energy colliders. In the SM {with a 125 GeV Higgs boson}, {the EWSB transition occurs via} a smooth cross-over rather than a FOPT~\cite{Kajantie:1996mn}. However, there are compelling theoretical arguments to expect new physics coupled to the SM Higgs not far from the TeV energy scale \cite{Ramsey-Musolf:2019lsf}. 
This could alter the nature of the {EWSB transition}, possibly making it {a first order  EWPT}. The existence of such a transition is a necessary ingredient for electroweak baryogenesis~\cite{Morrissey:2012db,Barrow:2022gsu,Asadi:2022njl} and could provide a source for observable gravitational radiation.

Two classes of collider probes of the new physics are possible. First, new particles could be produced at {some of} the new facilities, given that their reach in energy spans one/two orders of magnitude beyond the electroweak scale. 
Second, new physics coupled to the Higgs could lead to deviations $\delta_i$ of the Higgs couplings {or other properties} from their SM values---for example,
the Higgs trilinear self-coupling, $\lambda_{3}$ could be measured at $\delta_{\lambda_3} \sim 5 - 10 \%$ in future 100 TeV hadron colliders (e.g.~FCC-hh or SppC) and TeV scale lepton colliders; the Higgs-$Z$ boson coupling~\cite{Craig:2013xia,Huang:2016cjm} could be measured down to $\delta_{Zh} \sim 0.1 \%$ in future Higgs factories like ILC, CEPC or FCC-ee.
For more detail, see~\cite{Ramsey-Musolf:2019lsf, GW_EarlyUniv_WP} and references therein.
 
These two classes of collider probes of new EWSB physics, the direct production of the new particle states {and precision measurements of Higgs properties,} are complementary to each other and to the GW observation of the FOPT associated with the EWSB. As an example, we consider the model
where the EWPT is driven by interactions of a SM gauge singlet scalar with the Higgs. The singlet could be either real (\lq\lq xSM\,\rq\rq) and involve adding to the SM one new degree of freedom~\cite{Barger:2007im,Profumo:2007wc,Espinosa:2011ax,Profumo:2014opa,Huang:2016cjm}. Fig. \ref{fig:LHC_LISA_complementarity} shows the parameter space in this model: the collider probes and SGWB observations with the space-borne GW detector LISA explore the parameter space in this model in different, and hence complementary ways. The discovery of a GW signal from a phase transition in the early Universe could therefore guide searches for new physics at future colliders; conversely, new physics discovered at colliders could provide hints of early Universe phase transitions producing GW signals. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\hsize]{Figures/singlet_snr.pdf}
\end{center}
\caption{
EWPT strength $\alpha$ versus inverse duration (in Hubble units) $\beta/H^{*}$ 
for xSM benchmark scenarios. The orange benchmarks feature a singlet mixing 
$\left\vert\rm{sin}\,\theta \right\vert \gtrsim 0.1$, thus within reach of the HL-LHC, while the HL-LHC will not be able to probe the blue points (some of which are within reach of LISA). The red-orange-green curves correspond to the LISA sensitivity with a certain signal-to-noise  ratio (indicated in the figure). The black dashed lines correspond to constant values of $(\tau_{\text{sh}} H)^{-1}$, with $\tau_{\text{sh}} H < 1$ for the grey region. Figure adapted from~\cite{GW_EarlyUniv_WP}. 
}
\label{fig:LHC_LISA_complementarity}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    
Finally, we note that other (non-EW) phase transitions close to the weak scale can also leave both collider and GW signals. One of the well motivated scenarios is Supersymmetry. For example, the presence of light supersymmetric particles (such as stops or additional scalars in non minimal SUSY extensions) coupled to the SM Higgs could affect the properties of the EW symmetry breaking, rendering it strongly first order \cite{Carena:1996wj,Delepine:1996vn,Huang:2014ifa,Kozaczuk:2014kva,Huber:2015znp}. 

Futhermore, viable SUSY models should include a sector where SUSY is spontaneously broken, and SUSY breaking is tied to spontaneous R-symmetry breaking \cite{Nelson:1993nf}. One such study~\cite{Craig:2020jfv} has investigated under which conditions this transition can be first order, leading to a SGWB, demonstrating that the resulting GW spectrum covers the frequency range accessible to current and future GW detectors. Moreover, once the SUSY breaking mediation scheme is specified, the peak of the GW spectrum is correlated with the typical scale of the SM superpartners, and a visible GW signal would imply superpartners within reach of future colliders. 

\subsection{Topological Defects}

Phase transitions associated with symmetry breaking generically result in topological defects~\cite{Jeannerot:2003qv} that could have different forms~\cite{Kibble:1976sj,Vilenkin:2000jqa}. Three types of topological defects have been shown to produce SGWB: domain walls \cite{Vilenkin:1981zs,Sakellariadou:1990ne,Sakellariadou:1991sd,Gleiser:1998na,Hiramatsu:2010yz,Dunsky:2021tih}, textures \cite{Fenu:2009qf} and cosmic strings \cite{Vachaspati:1984gt,Blanco-Pillado:2017oxo,Blanco-Pillado:2017rnf,Ringeval:2017eww,Vilenkin:1981bx,Hogan:1984is,Siemens:2006yp,DePies:2007bm,Olmez:2010bi,Vachaspati:2015cma}. In all cases the amplitude of the GW signal grows with the symmetry breaking scale, implying that topological defects are effective probes of high energy physics. Furthermore, topological defects can also arise in superstring theories \cite{Sarangi:2002yt,Jones:2002cv,polchinski}, implying
that GW experiments can provide a novel and powerful way to test string theory~\cite{2006AAS...209.7413H,LIGOScientific:2017ikf}.

Among these, cosmic strings have been studied the most extensively, either as global strings (e.g. in axion dark matter models where a U(1) is broken to a vacuum with a discrete symmetry \cite{Chang:2019mza}) or as local strings in symmetry breaking chains that result from SO(10) breaking to the SM \cite{Dunsky:2021tih}. 
Considering all possible spontaneous symmetry breaking patterns from the GUT down to the SM gauge group, it was shown \cite{Jeannerot:2003qv} that cosmic string formation is unavoidable. 

Here we briefly highlight the SGWB production by local cosmic strings (for a more extensive discussion, see~\cite{GW_EarlyUniv_WP} and references therein).
Local strings with no internal structure can be described by the Nambu-Goto action, and are expected to quickly reach the scaling regime \cite{Kibble:1976sj}. The predicted SGWB spectrum is then defined by the dimensionless power spectrum for a string loop of a given length and by the number density of loops, both of which are studied in theoretical and numerical modeling~\cite{Blanco-Pillado:2017oxo,DV2,Ringeval:2017eww,Martins:1996jp,Martins:2000cs,Blanco-Pillado:2013qja,Blanco-Pillado:2011egf,Ringeval:2005kr,Lorenz:2010sm,Auclair:2019zoz}. The resulting SGWB spectrum is roughly constant over many decades of frequency, assuming standard cosmological history~\cite{Auclair:2019wcv}, as illustrated in Fig. \ref{fig:LHC_LISA_complementarity}. Detection of the SGWB due to cosmic strings could therefore be used to test for any departures from a standard cosmological picture \cite{Cui:2017ufi,Cui:2018rwi, Gouttenoire:2019kij}: probe new equations of state of the early universe, probe new particle species, and probe (pre-)inflationary universe~\cite{GW_EarlyUniv_WP}. Indeed, searches for cosmic string SGWB have already been conducted, placing upper limits on the string tension $G \mu \lesssim 9.6 \times 10^{-9}$ by LIGO-Virgo \cite{LIGOScientific:2021nrg}, and $G \mu \lesssim 10^{-10}$ by pulsar timing arrays \cite{Ellis:2020ena,Blanco-Pillado:2021ygr}. 
NANOGrav has reported a possible hint of cosmic strings \cite{NANOGrav:2020bcs}, although their observation may also be of instrumental origin.
Future experiments covering a wide frequency range will further improve the sensitivity to GW signals from cosmic strings, including Einstein Telescope, Cosmic Explorer, AEDGE, DECIGO, BBO, $\mu$Ares and Theia \cite{Punturo:2010zz,Yagi:2011wg,AEDGE:2019nxb,Hild:2010id,Sesana:2019vho,Theia:2017xtk}.
Cosmic string tension in the range of $G \mu \approx 10^{-16}- 10^{-15}$ or bigger could be detectable by LISA, with the galactic foreground affecting this limit more than the astrophysical background \cite{Boileau:2021gbr,Auclair:2019wcv}.


\subsection{Axion Like Particles}
% https://arxiv.org/pdf/1610.02743.pdf

Axions or axion-like particles (ALPs) are pseudo Nambu-Goldstone bosons that result from spontaneous symmetry breaking. Originally introduced to solve the strong CP problem, axions solve the hierarchy problem, inflation naturalness and naturally arise in string theory as modulus fields from dimensional compactification. Axions are typically light, and impact cosmology both at early and late times. Late-time effects of $\simeq 10^{-22}$ eV ALPs include the suppression of clustering of dark matter and galaxies, while $m_a <  10^{-27}$ eV ALPs generate late-time acceleration and change the amplitude of the Integrated Sachs Wolf (ISW) plateau in the CMB.

In the early universe, ALPs behave as relativistic species and can be mapped onto potential deviations from the Standard Model value of $N_\mathrm{eff}$, with deviations $\Delta N_\mathrm{eff}$ expected to be within the measurement sensitivity of experiments like CMB Stage IV \cite{cmbs4_sciencebook}.


If the axion symmetry-breaking occurs during inflation, ALPs would source isocurvature perturbations with an amplitude set by the energy scale of inflation, which also sets the amplitude of the tensor spectrum from GW. Upcoming polarization CMB measurements will constrain $H_I$ while complementary constraints from the temperature spectrum constrain the contribution of ALPs to the total cosmic energy budget. For ALPs in the $10^{-25} \, {\rm eV} < m_a < 10^{-24} \, {\rm eV}$ mass range,  current data allow a roughly $10\%$ contribution of ALPs to the total dark matter budget, with around a 1\% contribution to isocurvature and tensors. This will significantly improve in the coming decade with increases in sensitivity to CMB polarization. Alternatively, if the ULA U(1) symmetry is broken \textit{after the end} of inflation, a whitenoise power spectrum of isocurvature would be produced. For these models, the expected sensitivity of experiments like CMB-S4 is to axions with masses as `high' as $10^{-17}$ eV. 



%https://arxiv.org/pdf/2203.14915.pdf
%https://arxiv.org/pdf/2203.07064.pdf

